A Systematic Identification of Formal and Semi-formalLanguages and Techniques for Software-intensiveSystems-of-Systems Requirements Modeling

Software-intensive Systems-of-Systems (SoS) refer to an arrangement of managerially and operationally independent systems(i.e., constituent systems), which work collaboratively towards the achievement of global missions. Because some SoS are developed for critical domains, such as healthcare and transportation, there is an increasing need to attain higher quality levels, which often justifies additional costs that can be incurred by adopting formal and semi-formal approaches (i.e., languages and techniques) for modeling requirements. Various approaches have been employed, but a detailed landscape is still missing, and it is not well known whether they are appropriate for addressing the inherent characteristics of SoS. The main contribution of this article is to present this landscape by reporting on the state of the art in SoS requirements modeling. This landscape was built by means of a systematic mapping and shows formal and semi-formal approaches grouped from model-based to property-oriented ones. Most of them have been tested in safety-critical domains, where formal approaches such as finite state machines are aimed at critical system parts, while semi-formal approaches (e.g., UML and i*) address non-critical parts. Although formal and semi-formal modeling is an essential activity, the quality of SoS requirements does not rely solely on which formalism is used, but also on the availability of supporting tools/mechanisms that enable, for instance, requirements verification along the SoS lifecycle

==> Results_Conclusion.tex <==

%================================Milena Suggestion===========================
%
%\textcolor{red}{\section{Proposta para apresentação dos resultados}}

%\textbf{titulo do paper: "Languages for Expressing Systems-of-Systems Requirements: a Systematic Mapping"} OK, MUDAMOS

% \subsection{Languages for Modeling SoS Requirements}
% We identified X languages that have been used for modeling SoS requirements, namely: X, Y, Z, and K. <Aqui falar brevemente das que merecem mais destaque, as primeiras ou as mais consolidadas>. Following, we discuss N, M, .... which are currently used <falar que vai discutir aquelas que ainda "vivem", que tem uma comunidade ativa de desenvolvedores e praticantes/practictioners>. Cris, quais linguagens você acha mais relevantes?
% \blue{Milena e Elisa, aqui sugeria falar da SDL pois é de telecommunicação, fUML foi a unica aplicada a um sistema definido como SoS (S40 e S49 unicos que se definem como SoS), KAOS, por ter semi-formal and formal e pegar as mais usadas pelos estudos PVS, CSP, RSML, porque não tem nenhuma predominante. CONSIDERANDO USO HORIZONTAL}
%\blue{uso vertical entraria nas discusões}


%
%\subsubsection{Formal and semi-formal Languages} - changed

%\subsubsection{Formal and Semi-formal Techniques} changed
%
%Included studies SX, SY, SN used this language for ... It is also worth mentioning that this language was used with language X by SN, as they complement each other for....


%\textcolor{red}{FIM PROPOSTA}
%====================Milena Suggestion======================================

In this section, we present an overview of the results (in Section \ref{general_results}), answer RQ in Sections \ref{answers_rq1}, and finish with a discussion (Section \ref{discuss}). 


\subsection{General Results}\label{general_results}

In order to select the studies that performed requirements semi-formal and formal modeling, we considered the phases of \textit{analysis}, \textit{modeling\footnote{In selection of primary studies, we considered modeling as mathematical description of requirements and specification as the representation of these descriptions in model that will be checked by tool or graphical representation \cite{Nasa:1997FMS}, however, in description of this article used modeling to refer both, modeling and specification.}}, and \textit{specification} of a RE process and the selection was made based on in author's classification. 
The distinction fulfilled between the phases is somewhat unreal and therefore should not be taken integrally \cite{Nasa:1997FMS}.
In practice, to define these boundary is difficult and not instructive to identify with assurance where analysis ends and modeling begins, and consequently where modeling ends and specification begins \cite{Nasa:1997FMS, BaldwinDod:2008}.
We found similar difficulty when increase the abstraction level of RE process to life-cycle development, to identify where RE ends and Software Design begins.
These boundary, in both levels, become more difficult to identify in SoS context, which is constantly evolving with new requirements emerging that may influence the modeling and the models (i.e., specification) already specified. Inconsistency identified in verification phase, for example, may be trigger changes in all documentation as well as in whole life cycle development.

Despite of the challenges discussed (cf. \ref{background}) to formally and semi-formally model SoS requirements, efforts already have been destined in different perspectives to attempt to improve such activity.
An overview 


\begin{table*}[!ht]
    \caption{Characterization of the included primary studies}
    \label{tab:ComparativeTable}
    \centering
    \includegraphics[width=\linewidth]{ImagesModeling/OverviewLanguage1.pdf}
\end{table*}


%Often artificial it being difficult to identify the end of one and the beginning of the other and could not be performed so literally
Besides the challenges discussed in Section \ref{background} to formally and semi-formally model, verify, and validate SoS requirements, effort has been already destined in different perspectives to attempt to improve such activities.

As presented in Table \ref{tab:ComparativeTable}, the most effort has been applied in the modeling and verification of SoS requirements.
The former is addressed by all studies, and the latter by 61.5\% of them (i.e., 16 of 26 primary studies), and validation activity is adopted only in 15.4\% (i.e., 4 of 26 studies).

To improve the quality of requirements, after modeling the requirements, most of the studies performed their verification (i.e., S5, S8, S9, S19, S21, S27, S29, S30, S34, S43, S46, S47, and S49), other only the validation (i.e., S11), and others combine validation and verification of the SoS requirements (i.e., S1, S15, and S32).
This leaded us to infer the requirements quality is not only related to the techniques adopted to model or validate them, but also the verification done in the whole RE.

Moreover, not all studies that dealt with verification of SoS requirements explicitly described that their proposal were supported by automatic tools, although verification should be grounded by an automated support. Hence, while 16 studies addressed verification, 13 of them encompassed an automated support. With regard to validation, all studies (i.e., 4 or 15.4\%) mentioned to have an automated support.

Regarding the types of techniques adopted, the most studies used formal ones (i.e., 96.2\% or 25 studies).
This can be justified because the application domains addressed by the studies were critical and also because of certification regulations, such as DO278 \cite{EUROCAE:2002GCN} and ISO/DIS 26262 \cite{ISO26262:2009ROAD}, which require specific validation and/or verification procedure to the certification of these systems.
Besides that, 38.5\% (10 studies) adopted semi-formal languages or techniques, such as in S15 that used a graphical language for goal-oriented requirements engineering (i.e., KAOS) and the rules and symbolism of Linear Temporal Logic (LTL) to formally model requirements of a railway system. In general, it is worth highlighting that semi-formal techniques/languages have been mainly used to model non-critical parts of critical systems.
Additionally, informal technique (i.e., the manual inspection) was adopted by S8, together with a formal one, to evaluate the changes in requirements documents of a space shuttle system.

The most found application domains in the selected studies were railway (42.3\% or 11 studies),
natural disaster (3 studies), and avionics (2 studies).
Other diverse domains had only one study addressing them. In summary, we discovered that all application domains are critical, where failures could have no-desired results and, therefore, attention on the requirements adopting formal approaches to deal with requirements seems to be necessary.     
%no outro paper citar todos os domínios e estudos.



% \subsection{RQ1: Formal and Semi-formal Languages and Techniques for the SoS Requirements Modeling}\label{answers_rq1}

% Several formal and semi-formal languages and techniques have been established over time. Some of them are variants of another already existing as Timed-CSP, a variant of parallel language Communication Sequential Process (CSP) and are used to support the modeling or SoS requirements modeling. 
% We raised 18 languages used in 25 studies, 14 of them are formal and others four are semi-formal language, beyond of 14 techniques, six formal modeling  and type. These languages and techniques were represented in Figure \ref{fig:OverviewperYear} in a distribution over time.
% The brown balls shown define the years (from 1991 to 2017), the ball size indicates the quantity of study published in that year.
% For instance, in 2010, we have four studies (i.e., S27, S29, S30, and S31), because of this, the ball size in this year is bigger than 1991 that has only one (S1) study.
% Formal languages and techniques are represented in blue part and semi-formal in yellow part, besides modeling languages are showed in black color and modeling technique in red color.
% Let's return to example of the year 2010, in this year S29 and S30 used only a semi-formal language (UML-SD), S27 adopted just formal approaches being three languages (eXtensible Markup Language - XML, Web Service Definition Language - WSDL, and Web Service Business Process Execution Language - WSBPEL) and a technique (Finite State Machine - FSM), as well as S31 that used only formal technique fuzzy logic. 

% We also classify the formal and semi-formal languages and techniques considering some parameters (e.g., paradigm, specification type, and executable). This comparison was done in the light of specification styles described in \cite{Nasa:1997FMS, NasaSrivas:1995FVA, Lamsweerde:2000FSR, Ghezzi:2002}
% However, different terminologies were used in these studies for a same style, for example in technical report of NASA \cite{Nasa:1997FMS} is made the classification between model-oriented versus property-oriented. The first is a constructive style or prescriptive and the last is a declarative style or descriptive or also known as axiom -based.
% In order clarify our classification, we create the conceptual model presented in Figure \ref{fig:terminology} based in these studies that was our base of classification largest groups and also applied in parameter ``specification style'' together another information, such as documentation of the languages or techniques.

% \begin{figure*}[!ht]
%  	\centering
%  	\includegraphics[width=\linewidth]{ImagesModeling/SpecificationStyle.png}
%  	\caption{Conceptual model of specification style terminologies}
%  	\label{fig:terminology}
%  \end{figure*}
 
% The choice and use of specification style has a main role in systems requirements modeling mainly if the systems was critical as SoS, can be impact directly the abstraction level of the requirements specifications compromising all other phases of development.
% Model-based specification or constructive or prescriptive style describes the desired behavior for intending system, usually establishing models \cite{Ghezzi:2002}. They tends conduct to a specification more detail, with excess of specification, besides of necessary, which can allow vies at levels such as design and implementation \cite{NasaSrivas:1995FVA}. On the order hand, it is the easier style of understanding for no-technical user than Property-oriented style. 
% In this styles, i.e., Property-oriented specification or descriptive or declarative style, unlike the other, describes a desire properties of systems and encourages a specification with less detail and a more abstract specification \cite{Nasa:1997FMS, Ghezzi:2002}. Because of this, inconsistencies can be introduced with greater ease and can be less easily read and understood by the uninitiated reader than model-based specifications \cite{Nasa:1997FMS, NasaSrivas:1995FVA, Ghezzi:2002}. 
% Discussion considering trade-offs of specifications styles and their impacts in verification can be found in \cite{Nasa:1997FMS, NasaSrivas:1995FVA}.

% We classify the formal and semi-formal languages and techniques in two large groups: (i) model-based specification and (ii) property-based specification as depicts in Table XX.

% \begin{table*}[!ht]
%     \caption{Classification of formal and semi-formal languages and techniques based on specification style}
%     \label{tab:formalLcomparison}
%     \centering
%     \includegraphics[width=\linewidth]{ImagesModeling/ClassificationComparison1.pdf}
% \end{table*}


% In the two groups, subgroups were established based in the paradigm field of this table.  
% Moreover, we also considered other parameters, such as:
% (i) \textit{graphical model}: this parameters identify which languages or techniques may generate some graphical model.
% (ii) \textit{formal, semi-formal, languages}, and \textit{techniques}: by this parameters we raised the formal and semi formal languages and techniques. Languages are identified by black ball, while techniques by write ball.
% (iii) \textit{executable}:  executable specifications allow specifications be used as a ``prototype'', hence their can be minimize the time and significantly reduce the cost. Because of this, we classified the approaches in which their model is possible be executed.
% (iv) \textit{target}: this parameters identify the systems type described in their documentation and/or scientific documents (e.g., articles) of language or technique (e.g., large real-time system, systems-of-systems, and general systems)
% (v) \textit{available documentation}: we consider as available documentation when has more information, in addition to published scientific articles. For Example, f-UML has only article and Z language besides articles, has another documentations, as ISO/IEC13568:2002 \cite{ISO13568:2002Zlang}. 


Model-based specification is compound of five subgroups, object-oriented, state-based, event-based, agent-based, hybrid (i.e., in this group are one language (ModelicaML) and four techniques (statecharts, finite state machine, abstract state machine, and timed-automata-based fuzzy cognitive maps) that have more than one paradigm.).
In this style, object-oriented has important impact in systems development in consequently in requirements modeling using UML and their variants, such as SysML.
%UML was adopted by six studies (24\%) from 25 studies and SysML by one.
SysML and UML were used by S40 together ModelicaML, a derived of UML and SysML with graphical notation that facility several views, to model requirements of a SoS-cyber physical systems. 
In particular, SysML requirements diagram, block definition diagram, and internal block diagram were used in S19 combined with time petri nets and model checking to modeling and verify behavior requirements of a simple factory plant. 
Specific techniques of UML (i.e., activity diagram, class diagram, and sequence diagram) were also adopted for graphic representation of requirements in S19, S20, S29, S30, and S34. 
%S49 use a variant of UML called Fuzzy Unified Modeling Language - f-UML.
Although UML and SysML are the most recurrent for the development of object-oriented systems mainly in industry, they and their many variants such as executable UML (xUML\footnote{\url{https://xtuml.org/}}) do not present formal execution semantics to support formal modeling, V\&V; because of this, they are sometimes used combined with another formal approaches \cite{Haimes:2012}.
Semi-formal modeling like a descriptive style is easy to use and permits to quickly obtain a preliminary specifications of a systems, including their initial architecture, behavior and requirements aspects, but lack of formalization \cite{Linhares:2007IMV}.
On the order hand, formal modeling have formalization and the precision necessary to requirements modeling of critical and complex systems but requires some mathematical expertise.
A strategy usually applied is encapsulate the formal information in tools to specification, thereby the demand by mathematical expertise is minimized, the precision of the requirements specifications is maintained and can be improve adoption in the industry.
It is worth highlight that no formal language or technique have been used alone for SoS requirements modeling, besides of combination of formal and semi-formal approaches aforementioned, aggregation of more than one formal language, or language and technique have been used as well. 
For instance, S27 employed three formal languages (i.e., eXtensible Markup Language (XML), Web Service Business Process Execution Language (WSBPEL), and Web Service Definition Language (WSDL) and one formal method (Finite State Machine (FSM)) to establish a automata-based framework, which assist to improve the efficiency of verify a composite service to satisfies a specific group of non-functional requirements specified in WSDL.
This leads us to infer that SoS requirements modeling will not be done using only a formal modeling approach further a set of approaches that meet the challenges posed by the domain that will be modeled. Studies by domains of SoS could be more exploited, especially considering their main characteristics, such as evolutionary development and emergent behavior and evaluate which formal and/or semi-formal approaches provide support and assist better these characteristics.

Besides object-oriented, agent based (also known as goal-based) and state-based have been employed in industrial environments \cite{Nasa:1997FMS, Goldsby:2008GMD, Shamsaei:2013ASA, Piccolo:2015UFL}.
Agent-based is compound, in our SM, of two language i* framework and KAOS methodology.
Agents are active components, as human, devices, legacy software or software-to-be components that are responsible for achieving requirements and expectations \cite{RespectKAOS:2007}.
The i* framework is a conceptual modeling language and was adopted by S22, S26, and S39. Its main focus is to model the environment of the system-to-be, supporting critical modeling decision, such as identification of main goals of the systems, representation of multiple stakeholders and their interdependence, and possibilities towards these relationships \cite{Krishna:2009CPC, YuStar:2011}.
These characteristics can be interesting to the SoS development, as SoS are formed by the interoperability of independent constituents with different stakeholders and goals \cite{Bendov:2009,Maier:1998, Han:2013}.
KAOS Methodology adopted in S15, aside of agents, represent goals, which are desire systems properties expressed by stakeholders that will be meet by agents \cite{RespectKAOS:2007}. In general form, it is compound of four sub-models: (i) goal model: to form set of interrelated goal diagrams that have been put together for tackling a particular problem; (ii) object model: a diagram that includes objects (e.g., agents, entities, and relationships); (iii) responsibility model: this models describes which requirements and expectations each agent is responsible or assigned to it; and (iv) operation model: it receives all descriptions that an agent needs to accomplish the requirements \cite{Ponsard:2005EVV, RespectKAOS:2007}. 
KAOS assist in establishment of formal and semi-formal model. Semi-formal model is textual-based with graphical representation and a formalization is built on top of of this model. Besides that, it is possible formalize only part semi-formal model or whole model.
State-based paradigm may be considered the behavioral paradigm, since it is used to represent the systems behavior with their transitions states. In critical systems the modeling using behavior diagram, such as finite state machine and sequence diagram, have been employed in analysis of safety-critical systems not only in modeling, but also in verification by simulation means.
Simulation have been recurrently adopted in traditional approaches to evaluate the systems execution scenarios in design time and, more recently also applied to SoS \cite{Honour:2013, Neto:2014}. However, for SoS, simulation may require a great effort of engineering to reflect the performance issues, conflicting goals, standards, and emergent behavior (designed or unknown) \cite{Honour:2013, Zeigler:2015}. In spite of this, simulation presents important benefits, such as an early identification of errors and problems that need to be corrected before constructing in fact the SoS \cite{Neto:2014}.
State-based was used in 52\% of studies (i.e., S3, S5, S8, S9, S15, S21, S26, S27, S32, S35, S45, S46, and S49).
A example is S8 that used Prototype Verification System (PVS),  a language with tool and theorem prove integrated, with decision procedures for different theories including real and integer arithmetic in union with abstract state machine and TA-FCM. 
The S8 goal is to formalize the subsystems modeling of NASA's Space Shuttle using PVS exploring and documenting the feasibility and utility of formalizing critical Shuttle software requirements representing a spectrum of maturity levels. PVS still is actively used in NASA Langley Research Center (LaRC) applied PVS in several aerospace applications, such as pilot flying specification \cite{NasaCofer:2014DO333} and aerospace verification tool \cite{NasaWagner:2017Tool}.

Differently of model-based specification, property-based has only two groups, one with formal and semi-formal languages and techniques rules-based and another called ``Others'' that group the knowledge-based and XML-based.
Although, we have found few approaches property-based, they have been used widely used in requirements modeling \cite{Cordes:1988GRS, Nguyen:2014, abdalla:2015, NasaCofer:2014DO333}.
All languages (i.e., XML, WSDL, WSBPEL, Formal Language Maude (Maude), Modal Action Logic (MAL), and fuzzy description logic (f-DL)) and techniques (Interelement Requirements Diagram (IRD) and Fuzzy Logic) were applied only An example is Description logic ontology adopted by S49, f-SHIN used for describing the quality requirements, because it has strong ability of representation and decidability. 
Description logic are used as a formalism for representing knowledge and help to increase expressiveness without losing computational completeness, since all entailment are guaranteed to be computed, and decidability, which all computations has one time to finish, of reasoning systems \cite{Zou:2014VCT, Rossak:1994W3C:2018DL}.
In this context, f-UML language was established by authors of S49 to apply in SoS, its main focus is translating the capability needs into the high level requirements for SoS and evaluation the treatment this capability though of verification method that translate f-UML models into ontology specified in description logic, representing and verifying capability knowledge of SoS and consequently of the capabilities provides by constituent systems maintained quality, such as accuracy, flexibility, and facility of reuse of knowledge generate.

Due to SoS characteristics, there are significant challenges to create a verification environment able to manage SoS requirements.
Each constituent has its own verification responsibility, but each change in the constituent could result in verification events that could affect the entire SoS \cite{Honour:2013}.
Moreover, the managerial independence of the constituents often does not allow the synchronization of multiple life cycles.
Hence, verification of SoS requirements and systems, including integration testing, occurs sometimes without the presence of all constituents that compose the SoS (i.e., without all capabilities needs) \cite{Lewis:2009, Luna:2013}.
Besides that, as SoS has evolutionary development, modeling and verification of SoS requirements should be continuous, including evaluation of its capability considering its missions, which can impact considerably the knowledge representation of these systems and the verification process. \cite{Dahmann:2010} \cite{Honour:2013}.

\subsection{Discussion} \label{discuss}

The main objective of this article is to present a panorama of formal and semi-formal languages and techniques for SoS requirements modeling. 
Our investigations suggest that, formal and semi-formal modeling for SoS requirements is essential activities to developed these critical, complex, software-intensive systems and they require more rigour in requirements specifications process and consequently more formalism in their modeling and V\&V increasing the consistency, correctness, and completeness of the requirements and of the requirements specification document.
Similarly, industrial standards have also reinforce this necessity, mainly by means of certification of these systems, as the DO278 \cite{EUROCAE:2002GCN} used in certification of avionics, IEC/TR 80002 \cite{AAMI:2009MDS} used in medical device development, and EN 50126 \cite{EN50126:1999RAMS}; EN 50128 \cite{EN50128:2011RAMS} specify for railway applications.

Our SM draws on 26 studies, selected out of 4751, using a systematic process compound of several stages.
Of these, only 25 addresses some formal and semi-formal languages or techniques.
An important feature of our SM is that, though information search is make specifically to SoS domain, we did not narrow this in our search string, which allowed us search information in deeper into of the state-of-the-art about formal and semi-formal modeling of SoS requirements.
20 studies modeling part or all systems requirements using formal languages or techniques, five one adopted together formal and semi formal, and another nine combine more than one formal approach.
SoS have a inherent complexity in their development with new requirements emerging at runtime, a multiplicity of constituents systems, which will not always be known at design time or can change at runtime.
To model requirements of these systems certainly will be require the combination of more than one formal and/or semi-formal approach. To Apply formal modeling in all systems requirements will higher the cost development and time spent on specification, but minimize significantly errors introduced in another phases of the life cycles. On the order hand, modeling a systems only semi-formal methods reduce of time of specification, but increase the quantity of errors introduced in whole development process. The strategy adopted by industry is merge both, semi-formal and formal, as employed in S11, S15, S19, S20, and S26.

We identified 31 formal and semi-formal techniques and languages, of these only 18 are executable  and one language (i.e., XML) is interpreted, in other words, they are approaches that can be evaluated automatically, with support of tools. 
Tools can brings more precision in analysis and more accuracy to completeness, consistency, and correctness of requirements in modeling process in their verification. 
Besides that, of these 31 approaches 24 are well-documented, facilitating their application. However, the research field is relatively new to SoS, with publications concentrated in the last ten years.
Some publications of other domains, as embedded systems, cyber-physical systems, self-adaptive systems, were found presenting proposals that may be adapted to SoS.
A deeper analysis of how approaches have been applied to formally and semi-formally model and V\&V SoS requirements needs to be still conduced. This is because most of them were applied to similar systems and with characteristics compatible with SoS and not for real SoS. 
Of the 26 primary studies, only three (S40, S45, and S49) explicitly addressed these characteristics (i.e., managerial and/or operational independence, evolutionary development, emergent behavior, and geographical distribution \cite{Maier:1998, Lane:2013, Nielsen:2015}).
However, more attention still needs to be given to SoS requirements engineering activities, more specifically modeling and verification which are the activities that ensure the highest quality requirement at the end of the process. 
Tools that consider not only requirements at the SoS level, but that enable the elicitation and consequently modeling and verification of capabilities provided by the constituents need to be developed in a more integrated way.









%In our SM is noted that semi-formal and formal modeling and V\&V of SoS requirements are essential activities to developed of these systems (Repetido).
%However, the most of them are not studies applied in real world, and only three used simulation to validation considering the environment external. 
%Many studies have no critical parts modeling of systems, used semi-formal languages, such as UML and SySML and the most of them used state-based approach to model behavioral requirements. 

From of 25 studies, 15 of them modeling part or all systems requirements using formal languages and adopt 15 V\&V different formal methods and 18  V\&V tools.
As aforementioned, the research field is relatively new to SoS, with publications concentrated in the last ten years.
Some publications of other domains, as embedded systems, cyber-physical systems, self-adaptive systems, were found presenting proposals that may be adapted to SoS.
%Railway was the domain  used (i.e., 42.3\%), more specifically to the European and Chinese train control systems.
A deeper analysis of how approaches have been applied to formally and semi-formally model and validate SoS requirements needs to be still conduced. This is because most of them were applied to similar systems and with characteristics compatible with SoS and not for real SoS. 
Of the 26 primary studies, only three (S40, S45, and S49) explicitly addressed these characteristics (i.e., managerial and/or operational independence, evolutionary development, emergent behavior, and geographical distribution \cite{Maier:1998, Lane:2013, Nielsen:2015}).

It is noteworthy that despite the complexity of the systems, there is already the concern of integrated environments for modeling and V\&V, such as Telelogic Tau SDL Suit tool that allows modeling the generation of code and PVS that allows modeling and verification. 
However, more attention still needs to be given to SoS requirements engineering activities, more specifically modeling and verification which are the activities that ensure the highest quality requirement at the end of the process. 
Tools that consider not only requirements at the SoS level, but that enable the elicitation and consequently modeling and verification of capabilities provided by the constituents need to be developed in a more integrated way.

Furthermore, it can be noticed that modeling and V\%V positively contribute towards the quality of requirements; moreover, considering the activities of V\%V, the most applied one was verification.
This fact can be evidence that the quality is most related to the verification fulfilled in requirements, than only with their validation.
Note that, despite the importance of verification together with validation, from the 61.5\% of studies that adopted verification (16 studies), only 42.3\% of them (11 studies) were automatized, what can impact the accuracy, correctness, and consistency of the requirements of these systems.
Therefore, we believe that the identification of how formal and semi-formal approaches have been adopted to deal with SoS requirements, as well as an analysis involving verification approaches is also an important research topic, as it can contribute to provide new means to increase the quality of the entire SoS. 








\begin{table*}[!ht]
    \caption{\red{formal languages comparison  - completando}}
    \label{tab:formalLcomparison}
    \centering
    \includegraphics[width=\linewidth]{ImagesModeling/Formal_LanguagesDescription.pdf}
\end{table*}

%Timed-CSP evolve CPS notation allowing also a modeling of temporal aspects of sequencing and synchronization of real-time systems by insertion of operators, such as wait and timeout \cite{Davies:1995BHT}.

%According to NASA 1997: The advantages of a mature specification language are similar to those of a mature programming language: documentation is reasonably accessible and complete, tool support is available and generally reliable, there is a reasonably large body of associated literature and applications, and there is some measure of standardization so that a specification written in the language provides an unambiguous and generally accepted description.

%functional model: A functional model is one that employs the mathematical notion of function in a pure form, often in conjunction with an implicit and very simple computational model.

%ASMmodels: state machine model typically consists of an abstract representation of system state and a set of operations that manipulate the state to effect a transition from the current to the next state.

%On the other hand, if there is no need to reason about the evolution of the system over time,

%AutomataModel: Automata may be deterministic, meaning that there is a unique transition from a given state on a given input, or nondeterministic, meaning that there are zero, one, or more such transitions.

%OBJ-oriented model: Object-oriented models represent systems as structured collections of classes and objects with explicit notions of encapsulation, inheritance, and relations between objects.

%languages. Although mechanized support for formal systems is not discussed, one of the additional benefits of a high degree of formalization is that specifications written in a formal language are amenable to mechanical analysis and manipulation.

%FormalGraphica (RSML): These notations typically support an underlying methodology for specification and refinement. The challenge is to provide the benefits of a diagrammatic style with sufficient underlying formality to support a range of formal analysis techniques.


%\begin{table*}[!ht]
%    \caption{Formal and Semi-formal modeling languages for modeling SoS requirements}
%    \label{tab:modelingLanguage}
%    \centering
%    \includegraphics[width=\linewidth]{ImagesModeling/LanguagesTechComparison1.pdf}
%\end{table*}



\begin{table*}[!ht]
    \caption{\red{formal languages comparison  - completando}}
    \label{tab:formalLcomparison}
    \centering
    \includegraphics[width=\linewidth]{ImagesModeling/Formal_LanguagesDescription.pdf}
\end{table*}


\begin{table*}[!ht]
     \caption{\red{semi-formal languages comparison  - checar duas últimas colunas com Milena}}
    \label{tab:Semi-formalLcomparison}
    \centering
    \includegraphics[width=\linewidth]{ImagesModeling/Semi-formal_LanguagesDescription.pdf}
\end{table*}


%\begin{figure*}[!ht]
% 	\centering
% 	\includegraphics[width=\linewidth]{ImagesModeling/Formal_SemiformalByYear.png}
% 	\caption{Overview of the formal and semi-formal techniques and languages per year \red{Elisa, tentei fazer a legenda usado tamanho das bolas mas não ficou legal, então acho melhor descrever no texto}}
% 	\label{fig:OverviewperYear}
% \end{figure*}


\subsubsection{Formal and Semi-formal Techniques}

We identified 15 different formal languages used to model SoS requirements, as presented in Table \ref{tab:modelingLanguage}. In general, there is no predominant language (formal or semi-formal) in the selected studies. The most languages occur in one study and others were found in up to three studies.
In particular, Z language was used by S21, S26, and S35, following by CSP (Communicating Sequential Processes) used by two studies (S35 applied Timed-CSP and S43 used Hybrid CSP).
%---------------------xx-----------------------------------------

For instance, S35 used an object-oriented extension of Z language -- ZimOO -- to express, for example, complex data operations and differential (algebraic) equations to describe communication, concurrent, and real-time requirements \cite{Zhang:2012AOF}. Besides, S35 applied Timed-CSP, a mathematical approach that includes new operators like \textit{wait} and \textit{timeout} to the design and analysis of times of a distributed systems. 
%S35 used an object-oriented extension of Z language, ZimOO to express, for example, complex data operations and differential (algebraic) equations to describe communication, concurrent, and real-time requirements \cite{Zhang:2012AOF}, besides of timed-CPS a mathematical approach that includes new operators like \textit{Wait} and \textit{timeout} to the design and analysis of timed of a distributed systems \cite{Reed:1988TMC}.
In this case, a key factor is the communication among agents that can be made through timed Calculus of Communicating Systems (CCS) that have an operational semantics.
%Based in S35 is possible observe the communication process using CCS: a communication on \textit{k} described by \textit{k(t)w}, \textit{w} is restricted to happen in the closed time interval, and, after the communication, the variable \textit{t} holds the time at which it occurred (PARECE QUE É DETALHE DEMAIS QUE NÃO AJUDA NO TEXTO).
\red{Still in S35, Z language and Timed-CSP were used together with aspect-oriented approach (e.g., AspectZ) to model a real-time system in the railway domain.}
%Timed-CPS and Z language were used together with aspect-oriented approach (e.g., AspectZ) to modeling real-time systems (i.e., railway).

Hybrid-CSP is another extension of CSP that was adopted by S43, allowing continuous dynamics by introducing other elements, as differential equations, time constructs, and interruptions \cite{Chen:2015ETA}.
%Hybrid-CSP is another extension of CSP, allowing continuous dynamics by introduces others elements, as differential equations, time constructs, and interruptions \cite{Chen:2015ETA}.
Unlike Timed-CPS, a modification in Hybrid-CPS is to allow time-continuous evolution and not only time-discrete changes \cite{Maler:1991THS, Peleska:2004AFM}.
%Unliked Timed-CPS, an of the modifications in Hybrid-CPS is allows time-continuous evolution and not only time-discrete changes \cite{Maler:1991THS, Peleska:2004AFM}.
eXtensible Markup Language (XML), Web Service Business Process Execution Language (WSBPEL), and Web service definition language (WSDL) were adopted by S27 to establish an automata-based framework.
%eXtensible Markup Language (XML), Web Service Business Process Execution Language (WSBPEL), and Web service definition language (WSDL) were adopted by S27 to established an automata-based framework.

As S35 and S43, S49 employed different languages to model SoS requirements. In this case, S49 based on description logic and used Fuzzy Description Logic (f-DL) and Fuzzy Unified Modeling Language (f-UML).
%S49 also as S35 and S43 employ two different languages to modeling a SoS based on description logic (DL), Fuzzy Unified Modeling Language (f-UML) and Fuzzy description logic (f-DL).
A description logic is a knowledge representation language with a simple and well-established declarative semantics, usually decidable.
%=>> since have been designed and implemented efficient decision procedures to solve these problems CONSUFO ESSE FINAL.
Description logic expressivity and reasoning complexity can change according to mathematical constructors used in its establishment, i.e., a description logic can be general, spatial, temporal, spatiotemporal, and fuzzy \cite{Zou:2014VCT}.
%DL expressivity and reasoning complexity can change according to mathematical constructors used in its establishment, i.e., a DL can be general, spatial, temporal, spatiotemporal, and fuzzy \cite{Zou:2014VCT}.

Prototype Verification System (PVS) is a language with tool and theorem prove integrated, with decision procedures for different theories including real and integer arithmetic.
%Prototype Verification System (PVS) is a language with tool and theorem prover integrated, with decision procedures for different theories including real and integer arithmetic.
The goal of S8 is to formalize the modeling by using PVS and verification though of type checking, theorem prove, and proof obligation methods (cf. Table \ref{tab:Methods} or by applying the Stanford’s Mur$\phi$ Finite-state verification system tool, which is compound of a high level description language for finite-state asynchronous concurrent systems (cf. Table \ref{tab:tools}).
%The goals of S8 is formalizing modeling used PVS and verification though of type checking, theorem prover, and proof obligation methods (cf. Table \ref{tab:Methods} or by applied the Stanford’s Mur$\phi$ Finite-state verification system tool compound of a high level description language for finite-state asynchronous concurrent systems (cf. Table \ref{tab:tools}).
Similarly, S9 modeled requirements using PVS, made verification by means of parsing, but only type checking.
% Similarly, S9 models requirements used PVS, but make verification by means of parsing and only type checking.

Requirements State Machine Language (RSML) was adopted by S3 and S5 and both used it to model embedded systems. For graphical representation of the behavior state-based diagram, S3 adopted statecharts, whereas S5 used finite state machine (cf. Fig \ref{fig:semiformaltech}).
%Requirements State Machine Language (RSML) was adopted by S3 and S5 and both used RSML to modeling embedded systems and graphical representation of behavior state-based diagram, S3 represent is statecharts, whereas S5 in finite state machine (cf. Fig \ref{fig:semiformaltech}).
%Developed for Stanford Research Institute(SRI) international, PVS 
Other languages were adopted by only one study: S1 (Formal Language Maude \cite{SanchesAlonso:2012SCE}), S40 (ModelicaML \cite{Zhang:2014MLS}), and S32 (Specification and Description Language \cite{Yuan:2011MVS}). There are also studies that addressed temporal logic, such as S34 that applied Property Specification Language (PSL), an extension of Linear Temporal Logic (LTL) with UML to formalize of SoS requirements.

%=>> (i) S34 applied Property Specification Language (PSL), an extension of Linear Temporal Logic (LTL) with UML to formalize of SoS requirements; (ii) \red{OTHERS}.

%Other languages were adopted by only one study: Formal Language Maude \cite{SanchesAlonso:2012SCE}, ModelicaML \cite{Zhang:2014MLS}, and Specification and Description Language \cite{Yuan:2011MVS} and there are studies that addressed temporal logic as S34 that applied Property Specification Language (PSL) an extension of Linear temporal Logic (LTL) with UML to formalizing of SoS requirements.

With regard to semi-formal languages, we found four languages (cf. Table \ref{tab:modelingLanguage}): i* framework, KAOS Methodology, UML, and SysML.
The i* framework is an agent-oriented conceptual modeling language and was adopted by S22, S26, and S39. Its main focus is to model the environment of the system-to-be, supporting critical modeling decision, such as identification of main goals of the systems, representation of multiple stakeholders and their interdependence, and possibilities towards these relationships \cite{Krishna:2009CPC, YuStar:2011}.
%The i* framework is an agent-oriented conceptual modeling language and it was adopted by S22, S26, and S39. Its main focus is to model the environment of the system-to-be, supporting critical modeling decision, such as identification of main goals of the systems, representation of multiple stakeholders and their interdependence, and possibilities towards these relationships \cite{Krishna:2009CPC, YuStar:2011}.
These characteristics can be interesting to the SoS development, as SoS are formed by the interoperability of independent constituents with different stakeholders and goals \cite{Bendov:2009,Maier:1998, Han:2013}.

Regarding KAOS Methodology adopted in S15, aside of goals, agents represent an important type of KAOS concepts. Agents are active components, as human, devices, legacy software or software-to-be components that are responsible for achieving requirements and expectations \cite{RespectKAOS:2007}. In general form, it is compound of four sub-models: (i) goal model: to form set of interrelated goal diagrams that have been put together for tackling a particular problem; (ii) object model: a diagram that includes objects (e.g., agents, entities, and relationships); (iii) responsibility model: this models describes which requirements and expectations each agent is responsible or assigned to it; and (iv) operation model: it receives all descriptions that an agent needs to accomplish the requirements \cite{Ponsard:2005EVV, RespectKAOS:2007}.
%Aside of goals, agents represent an important type of KAOS concepts. Agents are active components, as human, devices, legacy software or software-to-be components that are responsible for achieving requirements and expectations \cite{RespectKAOS:2007}. In general form, it is compound of four sub-models: (i) goal model: to formed for setting of interrelated goal diagrams that have been put together for tackling a particular problem; (ii) object model: a diagram that include objects (e.g., agents, entities, and relationships); (iii) responsibility model: in this model is described for each agent, which requirements and expectations he is responsible or assigned to him; and (iv) operation model: it is receive all descriptions that an agent need to accomplish their requirements \cite{Ponsard:2005EVV, RespectKAOS:2007}.
%Informal technique (i.e., the manual inspection) was also adopted by S8 to evaluate the changes in requirements documents of space shuttle system.

SysML and UML were used by S40. In particular, SysML requirements diagram was used in S19 and specific techniques of UML (i.e., activity diagram, class diagram, and sequence diagram) were  adopted for graphic representation of requirements in S19, S20, S29, S30, and S34 (cf. Figure \ref{fig:semiformaltech}).
Although UML and SysML are the most recurrent for the development of object-oriented systems mainly in industry, they and their many variants such as executable UML (xUML\footnote{\url{https://xtuml.org/}}) do not present formal execution semantics to support formal modeling and validation; because of this, they are sometimes used in non-critical parts of the critical systems~ \cite{Haimes:2012}.
%não abordei novamente KAOS já falei demais dele la em cima. Elisa: Movi o KAOS para aqui nessa seção, mais acima.

Specifically regarding formal modeling techniques, Figure \ref{fig:formaltech} presents the main ones.
%Figure \ref{fig:formaltech} presents the main formal techniques applied in modeling of SoS requirements.
It is possible to observe that state-based techniques were the most used techniques, present in seven studies, i.e., in 27\% of them: in railway (S15, S32, and S46), avionics (S3 and S5), aerospace (S8), and natural disaster (S27).
%It is possible to observe that state-based model was the most used by the studies, mainly in railway (S15, S32, and S46) and avionics (S3 and S5) domain and it was addressed in seven studies (i.e., 27\% of them).
State-based techniques, such as finite state machine and statecharts, can be used to facilitate human understanding as well as to abstract real-world problems, keeping the high-level accuracy modeling \cite{Heimdahl:1996CCHS}.
%State-based techniques, such as finite state machine can be used to facilitate human understanding as well as to abstract real-world problems to given application domain, keeping the high-level accuracy modeling \cite{Heimdahl:1996CCHS}.

Fuzzy-based techniques were used in three studies: S31, S45, and S49.
%Fuzzy logic was used in three studies S31, S45, and S49.
In S31, it was used by means of Fuzzy Branching Temporal Logic (FBTL) to establish a new language (i.e., RELAX) to address uncertainty to self-adaptive systems requirements. It as evaluated in the smart home domain. 
In the similar perspective, S49 applied fuzzy to extend UML to model the vague, uncertain concepts of capacity of the SoS quality requirements, beyond specifying functional characteristics of SoS requirements as well.
Timed-Automata-Based Fuzzy Cognitive Maps (TA-FCMs) was adopted in S45.%=>> ISSO ESTÁ VAGO (esta faltando informação)
%In the first, it was used by means of fuzzy branching temporal logic (FBTL) to establish a new language (i.e., RELAX) to address uncertainty to self-adaptive systems requirements and evaluated in smart home domain.
%Timed-Automata-Based Fuzzy Cognitive Maps (TA-FCMs) and double-layered temporal granularity were adopted in the second study to modeling SoS requirements, and lastly, in the same perspective than S31, S49 also applied fuzzy to extend UML to model the vague, uncertain concepts of capacity of the SoS quality requirements, beyond specifying functional characteristics of SoS requirements as well.
%The CRAF language proposed in S49 was applied in the US Defense Department in C4ISR (Command, Control, Communication, Computer, Intelligence, Surveillance, and Reconnaissance) systems joint with 
Finally, Time Petri Nets was applied in S19 and S20. Both combine this technique with semi-formal languages (e.g., SysML and UML) to provide the necessary formalism to these languages to be applied in the modeling and verification of requirements of critical domains. 
%At the end, Time Petri nets was applied in S19 and S20, both combine it with semi-formal languages (e.g., SysML and UML) to provide the necessary formalism to these languages to be applied in the modeling and verification of requirements of critical domains. 
%Abstract state machine \cite{Crow:1998FSS} and other techniques were used only in a single study. (JÁ MENCIONADO LÁ EM CIMA)

%---------------------Milena Suggestion----------------------------


% \subsection{Methods and Tool Support for Validation and Verification of SoS Requirements}
% \subsubsection{Validation Methods}
% \subsubsection{Verification Methods}
% Subdividir em parágrafos (se nao for mto grande). 
% %
% Model checking... (mais comum). Studies N and Y use it for checking requirements expressed in languages W and H. Tool support is essential for applying model checking in industry, hence ... tools F and G have been used to verify these models, accordingly. 
% %
% Type checking...
% %
% DL inference engine... (tem bastante potencial de crescimento com o fortalecimento de ontologias e ferramentas)
% %
% Simulation... (qual dessas era esperada como mais comum? Seria interessante destacar esse ponto, era para ser mais utilizada, mas apenas um estudo aplica).


%\textcolor{red}{FIM PROPOSTA}

%--------------------Milena Suggestion --------------------------------------
\subsection{Discussion} \label{discuss}

%\section{Discussion}
%Discutir aqui qual parece ser a linguagem e o método mais promissor (se um usa o outro), em termos de popularidade e potencial de aplicação. Discutir que todos os estudos encontrados que utilizam uma notação formal ou semi-formal são para sistemas críticos, confirmando a "assumption" de que esses tipos de sistemas necessitam de formalismo. Contudo, é importante destacar que apenas uma parte dos requisitos necessita de tal formalismo, de modo que essas práticas precisam ser investigadas em conjunto com técnicas informais, que são altamente dependentes de linguagem natural.

The main objective of this paper is to present a panorama of the languages and techniques of modeling and methods and tools of V\&V for formally and semi-formally model, verify, and validate SoS requirements.
%The main objective of this paper is to present a panorama of the languages and techniques od modeling and methods and tools of V\&V for formally and semi-formally model, verify and validate SoS requirements.
Our investigations suggest that, formal and semi-formal modeling and validation for SoS requirements are essential activities to developed these critical, complex, software-intensive systems and they require more rigour in requirements specifications process and consequently more formalism in their modeling and V\%V, increasing the consistency, correctness, and completeness of the requirements and of the requirements specification document.
Similarly, industrial standards have also reinforce this necessity, mainly by means of certification of these systems, as the DO278 \cite{EUROCAE:2002GCN} used in certification of avionics, IEC/TR 80002 \cite{AAMI:2009MDS} used in medical device development, and EN 50126 \cite{EN50126:1999RAMS}; EN 50128 \cite{EN50128:2011RAMS} specify for railway applications.

Our SM draws on 26 studies, selected out of 4751, using a systematic process compound of several stages. 
An important feature of our SM is that, though information search is make specifically to SoS domain, we did not narrow this in our search string, which allowed us search information in deeper into of the state-of-the-arte about formal and semi-formal modeling and V\&validation of SoS requirements.

In our SM is noted that semi-formal and formal modeling and V\&V of SoS requirements are essential activities to developed of these systems.
However, the most of them are not studies applied in real world, and only three used simulation to validation considering the environment external. 
Many studies have no critical parts modeling of systems, used semi-formal languages, such as UML and SySML and the most of them used state-based approach to model behavioral requirements. 

From of 26 studies, 15 of them modeling part or all systems requirements using formal languages and adopt 15 V\&V different formal methods and 18  V\&V tools.
As aforementioned, the research field is relatively new to SoS, with publications concentrated in the last ten years.
Some publications of other domains, as embedded systems, cyber-physical systems, self-adaptive systems, were found presenting proposals that may be adapted to SoS.
%Railway was the domain  used (i.e., 42.3\%), more specifically to the European and Chinese train control systems.
A deeper analysis of how approaches have been applied to formally and semi-formally model and validate SoS requirements needs to be still conduced. This is because most of them were applied to similar systems and with characteristics compatible with SoS and not for real SoS. 
Of the 26 primary studies, only three (S40, S45, and S49) explicitly addressed these characteristics (i.e., managerial and/or operational independence, evolutionary development, emergent behavior, and geographical distribution \cite{Maier:1998, Lane:2013, Nielsen:2015}).

It is noteworthy that despite the complexity of the systems, there is already the concern of integrated environments for modeling and V\&V, such as Telelogic Tau SDL Suit tool that allows modeling the generation of code and PVS that allows modeling and verification. 
However, more attention still needs to be given to SoS requirements engineering activities, more specifically modeling and verification which are the activities that ensure the highest quality requirement at the end of the process. 
Tools that consider not only requirements at the SoS level, but that enable the elicitation and consequently modeling and verification of capabilities provided by the constituents need to be developed in a more integrated way.

Furthermore, it can be noticed that modeling and V\%V positively contribute towards the quality of requirements; moreover, considering the activities of V\%V, the most applied one was verification.
This fact can be evidence that the quality is most related to the verification fulfilled in requirements, than only with their validation.
Note that, despite the importance of verification together with validation, from the 61.5\% of studies that adopted verification (16 studies), only 42.3\% of them (11 studies) were automatized, what can impact the accuracy, correctness, and consistency of the requirements of these systems.
Therefore, we believe that the identification of how formal and semi-formal approaches have been adopted to deal with SoS requirements, as well as an analysis involving verification approaches is also an important research topic, as it can contribute to provide new means to increase the quality of the entire SoS. 


\section{Conclusions} \label{conclusion}

Formal and semi-formal modeling of SoS requirements can certainly contribute to improve the quality of these systems, when applied, mainly with verification.
In this scenario, the main contribution of this work was an panorama of languages and techniques for formally and semi-formally modeling requirements of SoS based also in similar systems.
As future work, besides of the needs already mentioned, we intend to perform a more specific investigation in this research area, for instance, as formal and semi-formal V\&V of SoS requirements have been treatment and integrated with modeling, beyond of consolidating and deepening the results of this SM, aiming at providing a more detailed analysis of each evidence presented in this work. 
Finally, we hope this work can call more attention of researchers and practitioners to the importance of adequately treating systems requirements modeling, mainly when such systems are the complex, critical, and software-intensive SoS.



% if have a single appendix:
%\appendix[Proof of the Zonklar Equations]
% or
%\appendix  % for no appendix heading
% do not use \section anymore after \appendix, only \section*
% is possibly needed

% use appendices with more than one appendix
% then use \section to start each appendix
% you must declare a \section before using any
% \subsection or using \label (\appendices by itself
% starts a section numbered zero.)
%


%\appendices
%\section{Proof of the First Zonklar Equation}

% you can choose not to have a title for an appendix
% if you want by leaving the argument blank
%\section{}
%Appendix two text goes here.


==> table_com_ID_49.tex <==
%============================Table=================== 
\begin{table*}[htb]
%\scriptsize
\centering
\caption{Primary studies included}
\vspace{0.1cm}
\label{tab:includedstudies}
\begin{tabular}{|p{0.4cm}|p{4.8cm}|p{10.4cm}|p{0.6cm}|}
\hline
\textbf{ID} & \textbf{Author}    &   \textbf{Title}                                                    & \textbf{Year} \\
\hline \hline
S1          & Atkinson, W. and Cunningham, J. &     \href{http://ieeexplore.ieee.org/document/73716/}{Proving properties of a safety-critical systems}                      & 1991          \\ \hline
S3          & Leveson, N.G. and Reese, J.D.      &  \href{http://ieeexplore.ieee.org/document/317428}{Requirements specification for process-control systems}            & 1994        \\ \hline
S5          & Heimdahl, M.P.E. and Leveson, N.G. &  \href{http://ieeexplore.ieee.org/document/508311/}{Completeness and consistency in hierarchical state-based requirements}              & 1996           \\ \hline
S8          & Crow, J. and Di Vito, B.           &  \href{https://dl.acm.org/citation.cfm?id=287023}{Formalizing Space Shuttle software requirements: four case studies}                & 1998       \\ \hline
S9          & Jong, E. et al.                         & \href{http://ieeexplore.ieee.org/document/839888/}{Refinement in requirements specification and analysis: a case study}               & 2000        \\ \hline
S11         & S\'anchez-Alonso, M. and Murillo, J. M. & \href{http://wer.inf.puc-rio.br/WERpapers/artigos/artigos\_WER02/alonson.pdf}{Specifying cooperation environment requirements using formal and graphical techniques}     & 2002  \\ \hline
S15         & Ponsard, C. et al.           &      \href{http://www.sciencedirect.com/science/article/pii/S1571066105050334}{Early verification and validation of mission critical systems}                         & 2005           \\ \hline
S19         & Linhares, M. V. et al.   &    \href{http://ieeexplore.ieee.org/document/4416788/}{Introducing the modeling and verification process in SysML}                                & 2007              \\ \hline
S20         & Ghazel, M. and El Koursi, E.M.  & \href{http://ieeexplore.ieee.org/document/4304240/}{Automatic level crossings: from informal functional requirements' specifications to the control model design}    & 2007   \\ \hline
S21         & Jamal, M. and Zafar, N.A.    &  \href{http://ieeexplore.ieee.org/document/4381340/}{Requirements analysis of air traffic control system using formal methods}                  & 2007              \\ \hline
S22         & Goldsby, H. J. et al.    & \href{http://ieeexplore.ieee.org/document/4492385/}{Goal-based modeling of dynamically adaptive system requirements}                              & 2008                \\ \hline
S26         & Krishna, A. et al.       & \href{http://ieeexplore.ieee.org/document/4492385/}{Consistency preserving co-evolution of formal specifications and agent-oriented conceptual models}   & 2009           \\ \hline
S27         & Sun, H. et al.           & \href{http://ieeexplore.ieee.org/document/5635065/}{Automata-based verification of security requirements of composite Web Services}                 & 2010                 \\ \hline
S29         & Tang, W. et al.              & \href{http://ieeexplore.ieee.org/document/5486079/}{Scenario-based modeling and verification for CTCS-3 system requirement specification}         & 2010               \\ \hline
S30         & Tang, W. et al.           &  \href{https://www.witpress.com/Secure/elibrary/papers/CR10/CR10069FU1.pdf}{Scenario-based modeling and verification of system requirement specification for the European Train Control System} & 2010    \\ \hline
S31         & Whittle, J. et al.    &  \href{https://link.springer.com/article/10.1007/s00766-010-0101-0}{RELAX: A language to address uncertainty in self-adaptive systems requirement}                 & 2010       \\ \hline
S32         & Yuan, L.  et al.   & \href{http://ieeexplore.ieee.org/document/5741283/}{Modelling and verification of the system requirement specification of train control system using SDL}    & 2011     \\ \hline
S34         & Cimatti, A. et al.  & \href{https://link.springer.com/article/10.1007/s10270-009-0130-7}{Formalizing requirements with object models and temporal constraints}                           & 2011               \\ \hline
S35         & Zhang, L.  & \href{https://ai2-s2-pdfs.s3.amazonaws.com/f558/42d4097e271e901622e5fed6ed1d6d22bfa0.pdf}{Aspect-oriented formal techniques of cyber physical systems}                                     & 2012                     \\ \hline
S39         & Deb, N. and Chaki, N.  & \href{http://ieeexplore.ieee.org/document/6785520/}{Verification of i* models for existential compliance rules in remote healthcare systems}         & 2014         \\ \hline
S40         & Zhang, L.   & \href{http://ieeexplore.ieee.org/document/6935460/}{Modeling large scale complex cyber physical control systems based on system of systems engineering approach}     & 2014     \\ \hline
S43         & Zou, L. et al.   & \href{https://link.springer.com/chapter/10.1007/978-3-642-54108-7\_14}{Verifying Chinese train control system under a combined scenario by theorem proving}             & 2014                 \\ \hline
S45         & Chen, Z. et al.   & \href{http://www.sciencedirect.com/science/article/pii/S2351978915002358}{Exploring a timed-automata fuzzy cognitive maps based approach for modeling systems of systems}  & 2015                 \\ \hline
S46         & Piccolo, A. et al.   &  \href{http://ieeexplore.ieee.org/document/7101503/}{Use of formal languages to represent the ERTMS/ETCS system requirements specifications}           & 2015           \\ \hline
S47         & Han, L. et al.   & \href{http://ieeexplore.ieee.org/document/7552030/}{Safety requirements specification and verification for railway interlocking systems}              & 2016                \\ \hline
S49         & Wang, Q.-L. et al. & \href{https://link.springer.com/article/10.1631/FITEE.1500309}{A quality requirements model and verification approach for system of systems based on description logic}  & 2017          \\ 
\hline
\end{tabular}
\end{table*}
%\end{sidewaystable*}
%=====================================xxx======================================================

